On Geometric Fourier Particle In Cell Methods

In this article we describe a unifying framework for variational electromagnetic particle schemes of spectral type, and we propose a novel spectral Particle-In-Cell (PIC) scheme that preserves a discrete Hamiltonian structure. Our work is based on a new abstract variational derivation of particle schemes which builds on a de Rham complex where Low's Lagrangian is discretized using a particle approximation of the distribution function. In this framework, which extends the recent Finite Element based Geometric Electromagnetic PIC (GEMPIC) method to a variety of field solvers, the discretization of the electromagnetic potentials and fields is represented by a de Rham sequence of compatible spaces, and the particle-field coupling procedure is described by approximation operators that commute with the differential operators in the sequence. In particular, for spectral Maxwell solvers the choice of truncated $L^2$ projections using continuous Fourier transform coefficients for the commuting approximation operators yields the gridless Particle-in-Fourier method, whereas spectral Particle-in-Cell methods are obtained by using discrete Fourier transform coefficients computed from a grid. By introducing a new sequence of spectral pseudo-differential approximation operators, we then obtain a novel variational spectral PIC method with discrete Hamiltonian structure that we call Fourier-GEMPIC. Fully discrete schemes are then derived using a Hamiltonian splitting procedure, leading to explicit time steps that preserve the Gauss laws and the discrete Poisson bracket associated with the Hamiltonian structure. These explicit steps share many similarities with standard spectral PIC methods. As arbitrary filters are allowed in our framework, we also discuss aliasing errors and study a natural back-filtering procedure to mitigate the damping caused by anti-aliasing smoothing particle shapes.

==> gempic_spectral_macros.tex <==
%% Macros for Gempic/Gemif papers
%
% legend for main math fonts:
%
% - vectors or vector-valued functions (with physical dimension > 1)
%   bold math font: prefix \b
%   \bE, \bB, \bLambda ...
%
% - arrays of stacked quantities (dim = numerical parameter)
%   bold sans-serif fonts: prefix \arr
%   \arrX, \arrE, \arrLambda ...
%
% - matrices & discrete operators between arrays
%   blackboard sans-serif: prefix \mat
%   \matM, \matJ ...
%
% - usual number sets
%   standard blackboard
%   \NN, \RR ...
%
% - functionals and some operators
%   caligraphic math: prefix \c
%   \cL, \cI ...


\usepackage[bbgreekl]{mathbbol}
\usepackage{amsmath,amssymb}
\usepackage{amsthm}  % added on 9.9.2020 -- no conflicts?
\usepackage{bm}
\usepackage{bbm}
\usepackage{upgreek}

\def\blankfirst{\phantom{V^0} }
\def\blanksecond{\phantom{ \{ } } %\hspace*{-5pt}}
\def\bbb{\phantom{\big|} }
\def\bBb{\phantom{\Big|} }

\def\mint{\int \mspace{-21.mu}\raise .8ex\hbox{\rotatebox{-80}{$|$}\,}}
\def\smint{\smallint \mspace{-13.mu}\raise -.1ex\hbox{\rotatebox{10}{--}}}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\rank}{rank}
\providecommand{\bproofof}[1]{\bigskip\noindent{\em Proof of #1.}~}
\def\bproof{\bigskip\noindent{\em Proof.}~}
\def\eproof{\hfill$\square$\nl}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

\def\ds{\displaystyle}
\def\nl{\newline}
\def\noi{\noindent}  %\ni = reverse \in

\def\<{\langle}
\def\>{\rangle}

\def\ie{{\em i.e. }}
\def\eg{{\em e.g. }}
\def\inc{{\rm in }}
%\newcommand\bm[1]{\bs {\rm #1}}

\def\h{\hat}
\def\wh{\widehat}
\def\t{\tilde}
\def\wt{\widetilde}
\def\u{\underline}
\def\Chi{\raise .3ex \hbox{\large $\chi$}} %\def\vp{\varphi}

\newcommand{\ii}{\ensuremath{\mathrm{i}}}

\def\ex{{\rm ex}}

\def\rmd{\, {\rm d}} %for integrals
\def\dd{\, {\rm d}} %for integrals also

\def\tb{\hbox{$\|\kern -.09em |$}}
\def\bigtb{\hbox{$\big\|\kern -.09em \big|$}}
\def\Bigtb{\hbox{$\Big\|\kern -.09em \Big|$}}
\newcommand\eref[1]{(\ref{#1})}

\def\GL{\mathbb{GL}}
\def\GO{\mathbb{GO}}

% macros for particle coordinates and grid nodes (to be changed if needed)
%
%\def\px{\bx}  % particle x, old
%\def\pv{\bv}  % particle v, old
\def\px{\bX}  % particle x, new
\def\pv{\bV}  % particle v, new

\def\pz{\bZ}  % particle variation, new
\def\py{\bY}  % particle w (var v), new

\def\gx{\bx}  % grid x

% macro for testing fields
\newcommand{\test}[1]{\check{#1}}


% blackboard fonts (eg for number sets)
% \mathbbm, \mathbbmss or \mathbbmtt with \usepackage{bbm}
\def\AA{\mathbbm{A}}
\def\BB{\mathbbm{B}}
\def\CC{\mathbbm{C}}
\def\DD{\mathbbm{D}}
\def\EE{\mathbbm{E}}
\def\FF{\mathbbm{F}}
\def\GG{\mathbbm{G}}
\def\II{\mathbbm{I}}
\def\JJ{\mathbbm{J}}
\def\KK{\mathbbm{K}}
\def\MM{\mathbbm{M}}
\def\NN{\mathbbm{N}}
\def\PP{\mathbbm{P}}
\def\QQ{\mathbbm{Q}}
\def\RR{\mathbbm{R}}
\def\SS{\mathbbm{S}}
\def\TT{\mathbbm{T}}
\def\UU{\mathbbm{U}}
\def\VV{\mathbbm{V}}
\def\WW{\mathbbm{W}}
\def\XX{\mathbbm{X}}
\def\YY{\mathbbm{Y}}
\def\ZZ{\mathbbm{Z}}

% black-board sans serif
% \mathbb require \usepackage ??  [bbgreekl]{mathbbol} of {upgreek} ??
\newcommand{\mat}[1]{\mathbb{#1}}
\def\matd{\mathbb{d}}
\def\matr{\mathbb{r}}
\def\matA{\mathbb{A}}
\def\matB{\mathbb{B}}
\def\matC{\mathbb{C}}
\def\matD{\mathbb{D}}
\def\matE{\mathbb{E}}
\def\matF{\mathbb{F}}
\def\matG{\mathbb{G}}
\def\matI{\mathbb{I}}
\def\matJ{\mathbb{J}}
\def\matK{\mathbb{K}}
\def\matM{\mathbb{M}}
\def\matN{\mathbb{N}}
\def\matO{\mathbb{O}}
\def\matR{\mathbb{R}}
\def\matS{\mathbb{S}}
\def\matT{\mathbb{T}}
\def\matt{\mathbb{t}}
\def\matW{\mathbb{W}}
\def\matw{\mathbb{w}}
\def\matZ{\mathbb{Z}}
\def\matLambda{\mathbb{\Lambda}}

\def\LaB{\mathbb{\Lambda}} %% ?? delete

% arrays of stacked quantities (dim = numerical parameter)
\newcommand{\arr}[1]{{\bm{\mathsf{#1}}}}
\newcommand\arre{{\bm{\mathsf{e}}}}
\newcommand\arrg{{\bm{\mathsf{g}}}}
\newcommand\arrB{{\bm{\mathsf{B}}}}
\newcommand\arrb{{\bm{\mathsf{b}}}}
\newcommand\arrD{{\bm{\mathsf{D}}}}
\newcommand\arrE{{\bm{\mathsf{E}}}}
\newcommand\arrU{{\bm{\mathsf{U}}}}
\newcommand\arrV{{\bm{\mathsf{V}}}}
\newcommand\arrW{{\bm{\mathsf{W}}}}
\newcommand\arrX{{\bm{\mathsf{X}}}}
\newcommand\arrY{{\bm{\mathsf{Y}}}}
\newcommand\arrZ{{\bm{\mathsf{Z}}}}
\newcommand\arrLambda{{\bm{\mathsf{\Lambda}}}}
\newcommand\arrsigma{{\bm{\mathsf{\sigma}}}}

% \newcommand\sfC{{\sf c}}
% \newcommand\sfE{{\sf e}}
% \newcommand\sfF{{\sf f}}
%
\newcommand\ttc{{\texttt{c}}}
\newcommand\tte{{\texttt{e}}}
\newcommand\ttf{{\texttt{f}}}

\newcommand\sfk{{\sf k}}
\newcommand\sfu{{\sf u}}
\newcommand\sfv{{\sf v}}
\newcommand\sfx{{\sf x}}
\newcommand\sfz{{\sf z}}

\newcommand\sfA{{\sf A}}
\newcommand\sfF{{\sf F}}
\newcommand\sfG{{\sf G}}
\newcommand\sfH{{\sf H}}
\newcommand\sfU{{\sf U}}
\newcommand\sfV{{\sf V}}
\newcommand\sfX{{\sf X}}

\def\Vsp{V}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cX{\mathcal{X}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}

\usepackage{mathrsfs}
\def\scrc{\mathscr{c}}
\def\scre{\mathscr{e}}
\def\scrf{\mathscr{f}}
\def\scrC{\mathscr{C}}
\def\scrE{\mathscr{E}}
\def\scrF{\mathscr{F}}
\def\scrP{\mathscr{P}}
\def\scrV{\mathscr{V}}

\newcommand\bfa{\mathbf{a}}
\newcommand\bfe{\mathbf{e}}
\newcommand\bfq{\mathbf{q}}
\newcommand\bfg{\mathbf{g}}
\newcommand\bfv{\mathbf{v}}
\newcommand\bfw{\mathbf{w}}
\newcommand\bfx{\mathbf{x}}
\newcommand\bfy{\mathbf{y}}
\newcommand\bfz{\mathbf{z}}

\newcommand\bfve{\mathbf{\ve}}

\newcommand\bfA{\mathbf{A}}
\newcommand\bfB{\mathbf{B}}
\newcommand\bfE{\mathbf{E}}
\newcommand\bfJ{\mathbf{J}}
\newcommand\bfK{\mathbf{K}}
\newcommand\bfU{\mathbf{U}}
\newcommand\bfV{\mathbf{V}}
\newcommand\bfW{\mathbf{W}}
\newcommand\bfX{\mathbf{X}}
\newcommand\bfY{\mathbf{Y}}
\newcommand\bfZ{\mathbf{Z}}

%\newcommand\x{\bx}
%\newcommand\hbx{{\hat \bx}}
\newcommand\uvec{{\be}}

\newcommand{\one}{\ensuremath{\mathbbm{1}}}

\def\bcP{ \boldsymbol{\mathcal{P}} }
\def\bcB{ \boldsymbol{\mathcal{B}} }

\def\Np{N_{\rm part}}

\def\Mf{\MM_{\rm f}}
\def\Mp{\MM_{\rm p}}
\def\Qp{\QQ_{\rm p}}

\def\ba{{\bs a}}
\def\bb{{\bs b}}
\def\bc{{\bs c}}
\def\be{{\bs e}}
\def\bj{{\bs j}}
\def\bk{{\bs k}}
\def\bsm{{\bs m}}
\def\bn{{\bs n}}
\def\bp{{\bs p}}
\def\bq{{\bs q}}
\def\br{{\bs r}}
\def\bu{{\bs u}}
\def\bv{{\bs v}}
\def\bw{{\bs w}}
\def\bx{{\bs x}}
\def\by{{\bs y}}
\def\bz{{\bs z}}

\def\bA{{\bs A}}
\def\bB{{\bs B}}
\def\bC{{\bs C}}
\def\bE{{\bs E}}
\def\bF{{\bs F}}
\def\bG{{\bs G}}
\def\bH{{\bs H}}
\def\bI{{\bs I}}
\def\bJ{{\bs J}}
\def\bK{{\bs K}}
\def\bL{{\bs L}}
\def\bM{{\bs M}}
\def\bN{{\bs N}}
\def\bP{{\bs P}}
\def\bQ{{\bs Q}}
\def\bR{{\bs R}}
\def\bS{{\bs S}}
\def\bV{{\bs V}}
\def\bW{{\bs W}}
\def\bX{{\bs X}}
\def\bY{{\bs Y}}
\def\bZ{{\bs Z}}

\def\obu{{\overline {\bs u}}}
\def\bpi{{\bs \pi}}
\def\bell{{\bs \ell}}
\def\btau{{\bs \tau}}
\def\bphi{{\bs \phi}}
\def\bvp{{\bs \vp}}
\def\bxi{{\bs \xi}}
\def\bpsi{{\bs \psi}}
\def\bsigma{{\bs \sigma}}
\def\bLambda{{\bs \Lambda}}
\def\bPi{{\bs \Pi}}
\def\bPhi{{\bs \Phi}}
\def\bnabla{{\bs \nabla}}

\def\u{\underline}

\def\uE{{\u \bE}}
\def\uB{{\u B}}
\def\urho{{\u \rho}}
\def\uJ{{\u \bJ}}

%\newcommand{\bu}{{\bf u}}
%\newcommand{\bv}{{\bf v}}
%\newcommand{\bw}{{\bf w}}

\def\bs{\boldsymbol}
\def\vp{{\varphi}}
\def\ve{{\varepsilon}}

\newcommand{\ee}{\ensuremath{\mathrm{e}}}

\def\Ampere{{Amp\`{e}re}}


%\def\h{{\rm h}}
%\def\c{{\rm c}}
%\def\nc{{\rm nc}}

\def\Dt{{\Delta t}}

\def\dt{{\partial_{t}}}
\def\dtt{{\partial^2_{t}}}
\def\dx{{\partial_{x}}}
\def\dy{{\partial_{y}}}
\def\dxx{{\partial^2_{x}}}
\def\dxy{{\partial^2_{xy}}}
\def\dyy{{\partial^2_{yy}}}
\def\dv{{\partial_{v}}}

\def\dtheta{{\partial_{\theta}}}
\def\dr{{\partial_{r}}}

\def\pa{\partial}
\def\opa{{\overline \pa}}


\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sinc}{sinc}

\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\Ker}{Ker}
%\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\Ima}{Im}

%\DeclareMathOperator{\strikedcurl}{{\rm \sout{curl}}}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\bcurl}{{\bf curl}}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\bgrad}{{\bf grad}}

\DeclareMathOperator{\DivSC}{\textsc{div}}
\DeclareMathOperator{\curlSC}{\textsc{curl}}
\DeclareMathOperator{\gradSC}{\textsc{grad}}

%\DeclareMathOperator{\bnabla}{{\bs \nabla}}


\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\bigabs}[1]{\big|#1\big|}
\providecommand{\Bigabs}[1]{\Big|#1\Big|}
\providecommand{\Abs}[1]{\left\lvert#1\right\rvert}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\bignorm}[1]{\big\|#1\big\|}
\providecommand{\Bignorm}[1]{\Big\|#1\Big\|}
\providecommand{\Norm}[1]{\left\lVert#1\right\rVert}

\providecommand{\tnorm}[1]{\tb#1\tb}
\providecommand{\bigtnorm}[1]{\bigtb#1\bigtb}
\providecommand{\Bigtnorm}[1]{\Bigtb#1\Bigtb}

\providecommand{\sprod}[2]{\langle#1,#2\rangle}
\providecommand{\bigsprod}[2]{\big\langle#1,#2\big\rangle}
\providecommand{\Bigsprod}[2]{\Big\langle#1,#2\Big\rangle}

\providecommand{\diff}[2]{\frac{\delta #1}{\delta #2}}
\providecommand{\Dx}{{\Delta x}}

\newcommand{\fdt}{\frac{\partial }{\partial t}}

\providecommand{\range}[2]{\llbracket #1, #2 \rrbracket}
\providecommand{\Range}[2]{\left\llbracket #1, #2 \right\rrbracket}



%colors -- see doc at http://repositorios.cpai.unb.br/ctan/macros/latex/contrib/xcolor/xcolor.pdf
% \usepackage[svgnames]{xcolor} -- already imported by beamer class
\providecommand{\blue}[1]{{\color{Blue} #1}}
\providecommand{\green}[1]{{\color{Green} #1}}
\providecommand{\red}[1]{\textcolor{Red}{#1}}
\providecommand{\purple}[1]{{\color{Purple} #1}}
\providecommand{\orange}[1]{\textcolor{Orange}{#1}}


% \definecolor{azure}{rgb}{0.0, 0.5, 1.0}
% \definecolor{blue(ryb)}{rgb}{0.01, 0.28, 1.0}

% \providecommand{\red}[1]{\textcolor{red!90!fg}{#1}}
% %\providecommand{\blue}[1]{\textcolor{blue!80!fg}{#1}}
% %\providecommand{\blue}[1]{\textcolor{azure}{#1}}
% \providecommand{\blue}[1]{\textcolor{blue(ryb)}{#1}}
% \providecommand{\green}[1]{\textcolor{green!50!fg}{#1}}
% \providecommand{\gray}[1]{\textcolor{black!50!bg}{#1}}

% \def\ra{\blue{$\rightsquigarrow~$}} %$\rightarrow$

% \providecommand{\darkblue}[1]{\textcolor{blue!65!fg}{#1}}

\DeclareRobustCommand{\katharina}[1]{\textcolor{red}{(Katharina: #1)} } %{\begingroup\sethlcolor{red}\hl{(Katharina:) #1}\endgroup} }
\providecommand{\martin}[1]{\textcolor{purple}{(Martin: #1)}}
\providecommand{\eric}[1]{ \textcolor{blue}{Eric: #1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HIDE command :
% (see below)
%

\newcommand\hide[1]{

\bigskip
{\bf Hidden computations:
[ written for completeness, see \texttt{$\backslash$hide} command in header]:}
\nl\nl
#1
\nl\nl
{\bf End of hidden computations
[see \texttt{$\backslash$hide} command in header]:}
\nl
}

%
% Uncomment below to really hide the additional computations
%

%\renewcommand\hide[1]{}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\todo}[1]{{\bf [[ Todo: #1]]}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Added for strong Ampere

\newcommand{\Lab}{\ensuremath{\boldsymbol{\Lambda}}}

% \newcommand{\X}{\ensuremath{\mathbf{X}}}
% \newcommand{\V}{\ensuremath{\mathbf{V}}}
% \newcommand{\U}{\ensuremath{\mathbf{U}}}
% > redundant with \bfX, \bfV, \bfU

\newcommand{\ham}{\ensuremath{\mathcal{H}}}

\newcommand{\fracd}[2]{\ensuremath{\frac{\delta   #1}{\delta   #2}}}
\newcommand{\fracp}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
%\newcommand{\dd}{\ensuremath{\mathrm{d}}}
\newcommand{\iz}[1]{\ensuremath{I^0_{h,\uvec_#1}}}
\newcommand{\io}[1]{\ensuremath{I^1_{h,\uvec_#1}}}
\newcommand{\itwo}[1]{\ensuremath{I^2_{h,\uvec_#1}}}
\newcommand{\DDd}{\ensuremath{D}}
\newcommand{\cbra}[2]{\ensuremath{\left \{ #1 , #2 \right \}}}

